LeGO: Leveraging a Surface Deformation Network for Animatable Stylized Face Generation with One Example

Recent advances in 3D face stylization have made significant strides in few to zero-shot settings. However, the degree of stylization achieved by existing methods is often not sufficient for practical applications because they are mostly based on statistical 3D Morphable Models (3DMM) with limited variations. To this end, we propose a method that can produce a highly stylized 3D face model with desired topology. Our methods train a surface deformation network with 3DMM and translate its domain to the target style using a paired exemplar. The network achieves stylization of the 3D face mesh by mimicking the style of the target using a differentiable renderer and directional CLIP losses. Additionally, during the inference process, we utilize a Mesh Agnostic Encoder (MAGE) that takes deformation target, a mesh of diverse topologies as input to the stylization process and encodes its shape into our latent space. The resulting stylized face model can be animated by commonly used 3DMM blend shapes. A set of quantitative and qualitative evaluations demonstrate that our method can produce highly stylized face meshes according to a given style and output them in a desired topology. We also demonstrate example applications of our method including image-based stylized avatar generation, linear interpolation of geometric styles, and facial animation of stylized avatars.

==> figure_tex/figure_A0.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/figure_A0.png}
\caption{Detailed illustration of $L_{in}$ and $L_{across}$ with hierarchical rendering. The blue box shows an example of the predefined pivots of hierarchical rendering.}
\vspace{-2pt}
\label{fig:mtg}
\end{figure}

==> figure_tex/figure_A1.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/figure_A1.pdf}
\caption{First two rows are identity exemplar mesh and style exemplar mesh in our dataset, created for fine-tuning. Last row shows deformation target meshes for experiments}
\vspace{-4pt}
\label{fig:dataset}
\end{figure}

==> figure_tex/figure_B0.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{figures/figure_B0.png}
\caption{Visualization of deformation network in detail.}
\label{fig:deformationnet}
\end{figure*}

==> figure_tex/figure_B1.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=1.05\linewidth]{figures/figure_B1.pdf}
\caption{Artifacts occurred by simple displacement transfer. The red boxes show the close-up views. The boxes colored in red show the result of simple dispacement with artifacts(sunk nose and penetration on eye region) unlike Ours, colored in black.}
\label{fig:naiive}
\end{figure}

==> figure_tex/figure_C1.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{figures/C11.png}
\caption{Comparison with NFR and LEGO. Becaus NFR is designed for expression transfer, it's expression encoder cannot preserve identity.}
\label{fig:nfr}
\end{figure*}

==> figure_tex/figure_C2.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{figures/C0.pdf}
\caption{Comparison with Ours and Ours w. direct $L_{style}$. Both methods generated the style well while Ours followed the expression from the deformation target better compared to Ours w. direct $L_{style}$.}
\vspace{-4pt}
\label{fig:animation}
\end{figure*}

==> figure_tex/figure_D0.tex <==
\begin{figure}[h]
\centering
\vspace{-4pt}
\includegraphics[width=\linewidth]{figures/figure_D0.png}
\caption{Additional results of style interpolation.}
\vspace{-6pt}
\label{fig:interpolation}
\end{figure}

==> figure_tex/figure_D1.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.75\linewidth]{figures/figure_D1.png}
\vspace{-8pt}
\caption{Retargeting from video, two different styles are shown for each input. Left examples are from Talking-head-1KH~\cite{wang2021facevid2vid} and right examples are from MEAD dataset~\cite{wang2020mead}.}
\vspace{-10pt}
\label{fig:video}
\end{figure*}

==> figure_tex/figure_E0.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.88\linewidth]{figures/figure_E0.png}
\caption{Additional results on all 8 different styles.}
\vspace{-5pt}
\label{fig:add1}
\end{figure*}

==> figure_tex/figure_E1.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.88\linewidth]{figures/figure_E1.png}
\caption{Additional results on all 8 different styles.}
\vspace{-5pt}
\label{fig:add2}
\end{figure*}

==> figure_tex/figure_E2.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.88\linewidth]{figures/figure_E2.png}
\caption{Additional results on all 8 different styles.}
\vspace{-5pt}
\label{fig:add3}
\end{figure*}

==> figure_tex/figure_teaser.tex <==
\begin{center}
    %\setlength{\tabcolsep}{0.12cm}
    %\setlength{\itemwidth}{5.2cm}
    \begin{tabular}{c}
        \includegraphics[width=1\linewidth,natwidth=610,natheight=642]{figures/teaser.pdf}
    \end{tabular}
    \vspace{-2mm}
    \captionof{figure}{{(a) The proposed method demonstrates robustness to unseen face identities and topologies and effectively generates stylized output faces with desired topologies. (b) Our stylized avatars can be animated using 3DMM blend shapes.}}
    \label{teaser}
\end{center}
